Renmin University of China at TRECVID 2022: Improving Video Search by Feature Fusion and Negation Understanding

We summarize our TRECVID 2022 Ad-hoc Video Search (AVS) experiments. Our solution is built with two new techniques, namely Lightweight Attentional Feature Fusion (LAFF) for combining diverse visual / textual features and Bidirectional Negation Learning (BNL) for addressing queries that contain negation cues. In particular, LAFF performs feature fusion at both early and late stages and at both text and video ends to exploit diverse (off-the-shelf) features. Compared to multi-head self attention, LAFF is much more compact yet more effective. Its attentional weights can also be used for selecting fewer features, with the retrieval performance mostly preserved. BNL trains a negation-aware video retrieval model by minimizing a bidirectionally constrained loss per triplet, where a triplet consists of a given training video, its original description and a partially negated description. For video feature extraction, we use pre-trained CLIP, BLIP, BEiT, ResNeXt-101 and irCSN. As for text features, we adopt bag-of-words, word2vec, CLIP and BLIP. Our training data consists of MSR-VTT, TGIF and VATEX that were used in our previous participation. In addition, we automatically caption the V3C1 collection for pre-training. The 2022 edition of the TRECVID benchmark has again been a fruitful participation for the RUCMM team. Our best run, with an infAP of 0.262, is ranked at the second place teamwise.

==> table-all-models.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[tb!]
\renewcommand{\arraystretch}{1.2}
  \centering
  \caption{\textbf{Varied models used in our experiments}. A model  postfixed with the letter \emph{b} indicates that the model is pre-trained on the GCC dataset. As GCC is an image collection, it cannot be used to pre-train models that uses the C3D feature.}
    \begin{tabular}{lllllc}
    \toprule
    \textbf{Model} & \textbf{Network} & \textbf{Sentence Encoders} & \textbf{Video Features} & \textbf{Pre-training}  \\
\midrule
    1     & W2VV++ & BoW   & ResNet+ResNeXt & $\times$ \\
    1b    & W2VV++ & BoW   & ResNet+ResNeXt & $\surd$   \\
    1c    & W2VV++ & BoW   & ResNet+ResNeXt+C3D & $\times$ \\
    \cmidrule{1-5}
    2     & W2VV++ & NetVlad & ResNet+ResNeXt & $\times$        \\
    2b    & W2VV++ & NetVlad & ResNet+ResNeXt & $\surd$   \\
    2c    & W2VV++ & NetVlad & ResNet+ResNeXt+C3D & $\times$        \\
    \cmidrule{1-5}
    3     & SEA   & BoW, NetVlad & ResNet+ResNeXt & $\times$        \\
    3b    & SEA   & BoW, NetVlad & ResNet+ResNeXt & $\surd$   \\
    3c    & SEA   & BoW, NetVlad & ResNet+ResNeXt+C3D & $\times$        \\
    \cmidrule{1-5}
    4     & SEA   & BoW, w2v & ResNet+ResNeXt & $\times$        \\
    4b    & SEA   & BoW, w2v & ResNet+ResNeXt & $\surd$   \\
    4c    & SEA   & BoW, w2v & ResNet+ResNeXt+C3D & $\times$       \\
    \cmidrule{1-5}
    5     & SEA   & BoW, w2v, bi-GRU & ResNet+ResNeXt & $\times$       \\
    5b    & SEA   & BoW, w2v, bi-GRU & ResNet+ResNeXt & $\surd$   \\
    5c    & SEA   & BoW, w2v, bi-GRU & ResNet+ResNeXt+C3D & $\times$      \\
    \cmidrule{1-5}
    6     & SEA   & BoW, w2v, bi-GRU, BERT & ResNet+ResNeXt & $\times$       \\
    6b    & SEA   & BoW, w2v, bi-GRU, BERT & ResNet+ResNeXt & $\surd$   \\
    6c    & SEA   & BoW, w2v, bi-GRU, BERT & ResNet+ResNeXt+C3D & $\times$    \\
%     1     & W2VV++ & BoW   & ResNet+ResNeXt & $\times$       \\
%     2     & W2VV++ & NetVlad & ResNet+ResNeXt & $\times$        \\
%     3     & SEA   & BoW, NetVlad & ResNet+ResNeXt & $\times$        \\
%     4     & SEA   & BoW, w2v & ResNet+ResNeXt & $\times$        \\
%     5     & SEA   & BoW, w2v, bi-GRU & ResNet+ResNeXt & $\times$       \\
%     6     & SEA   & BoW, w2v, bi-GRU, BERT & ResNet+ResNeXt & $\times$       \\
% \cmidrule{2-5}    
%     7     & W2VV++ & BoW   & ResNet+ResNeXt & $\surd$ &  \\
%     8     & W2VV++ & NetVlad & ResNet+ResNeXt & $\surd$ &  \\
%     9     & SEA   & BoW, NetVlad & ResNet+ResNeXt & $\surd$ &  \\
%     10    & SEA   & BoW, w2v & ResNet+ResNeXt & $\surd$ &  \\
%     11    & SEA   & BoW, w2v, bi-GRU & ResNet+ResNeXt & $\surd$ &  \\
%     12    & SEA   & BoW, w2v, bi-GRU, BERT & ResNet+ResNeXt & $\surd$ &  \\
% \cmidrule{2-5}    
%     13    & W2VV++ & BoW   & ResNet+ResNeXt+C3D & $\times$      &  \\
%     14    & W2VV++ & NetVlad & ResNet+ResNeXt+C3D & $\times$      &  \\
%     15    & SEA   & BoW, NetVlad & ResNet+ResNeXt+C3D & $\times$      &  \\
%     16    & SEA   & BoW, w2v & ResNet+ResNeXt+C3D & $\times$      &  \\
%     17    & SEA   & BoW, w2v, bi-GRU & ResNet+ResNeXt+C3D & $\times$     &  \\
%     18    & SEA   & BoW, w2v, bi-GRU, BERT & ResNet+ResNeXt+C3D & $\times$     &  \\
    \bottomrule

    \end{tabular}%
  \label{tab:all-models}%
\end{table*}%


==> table-compare-rerank.tex <==
\begin{table} [htbp!]
\renewcommand{\arraystretch}{1}
\caption{\textbf{Comparing the influence of rerank on the TRECVID 16-21 AVS tasks}. }

\label{tab:compare-rerank}
\centering
 \scalebox{0.7}{
 \begin{tabular}{@{} llrrrrrrrr @{}}
\toprule
\textbf{Model} & \multicolumn{1}{l}{\textbf{TV16}} & \multicolumn{1}{l}{\textbf{TV17}} & \multicolumn{1}{l}{\textbf{TV18}} & \multicolumn{1}{l}{\textbf{TV19}} & \multicolumn{1}{l}{\textbf{TV20}} & \multicolumn{1}{l}{\textbf{TV21}} & \multicolumn{1}{l}{\textbf{MEAN}} \\
\hline
LAFF & 0.262 & 0.357 & 0.193 & 0.243 & 0.357 & 0.363 & 0.296 \\
LAFF+Rerank & 0.276 & 0.361 & 0.192 & 0.255 & 0.361 & 0.365 & 0.302\\
 % \hline
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}

==> table-select-2dfeat.tex <==
% \begin{table*} [tb!]
% \renewcommand{\arraystretch}{1}
% \caption{\textbf{Performance of our four runs and  the individual models on the TRECVID 2016--2020 AVS tasks}.}

% \label{tab:avs-seclet-single}
% \centering
%  \scalebox{1}{
%  \begin{tabular}{@{} l lllll l l l  @{}}
% \toprule

% Run & Model &\textbf{TV16} & \textbf{TV17} &\textbf{TV18} &\textbf{TV19} & \textbf{TV20} & \textbf{TV21}& \textbf{MEAN} \\
%  \hline
% 1 & \emph{Late fusion of Run3, Run4, CLIP} &0.246  &0.320  &0.161  & 0.227 & 0.366 & 0.343 &0.277  \\
% 2 & \emph{MEA-rerank} & 0.224 & 0.342 & 0.168 & 0.224 & 0.361 & 0.340 & 0.293 \\
% 3 & \emph{MEA} & 0.223 & 0.342 & 0.167 & 0.223 & 0.361 & 0.340 & 0.292 \\
% 4 & \emph{SEA-clip} & 0.232	&0.255	&0.135 & 0.213 & 0.358 & 0.337 &0.239 \\

% \bottomrule
% \end{tabular}
%  }% end of scalebox
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht!]
\caption{\textbf{Comparing 2D and 3D visual features on the TRECVID 19/20 AVS task}. Training data: MSR-VTT + TGIF.}
\centering
\setlength{\tabcolsep}{1.6mm}
\scalebox{1}{
    %  \small 
\begin{tabular}{clrrr}
\toprule

\multicolumn{1}{l}{\textbf{Rank}} & \textbf{Visual features} & \multicolumn{1}{c}{\textbf{TV19}} & \multicolumn{1}{c}{\textbf{TV20}} & \multicolumn{1}{c}{\textbf{MEAN}} \\
\hline
\multicolumn{5}{l}{\textbf{\textit{Retrieval model}: SEA-clip \cite{ChenHu2021} }} \\
1 & \textit{rx101-wsl-clip} &  0.204 & 0.262 & 0.233\\
2 & \textit{rx101-re152-clip} & 0.199 & 0.249 & 0.224 \\
\multicolumn{5}{l}{\textbf{\textit{Retrieval model}: SEA(bow, w2v) \cite{tmm21-sea}  }} \\
3 & \textit{rx101-re152-clip} & 0.199 & 0.233 & 0.216 \\
4 & \textit{rx101-wsl-clip} & 0.183 & 0.239 & 0.211 \\
5 & \textit{rx101-clip} & 0.196 & 0.223 & 0.210 \\
6 & \textit{rx101-re152-wsl-clip} & 0.182 & 0.238 & 0.210 \\
7 & \textit{rx101-re152-wsl} & 0.159 & 0.208 & 0.184 \\
8 & \textit{rx101-re152} & 0.167 & 0.201 & 0.184 \\
9 & \textit{rx101-wsl} & 0.148 & 0.208 & 0.178 \\
10 & \textit{clip-wsl} & 0.148 & 0.208 & 0.178 \\
11 & \textit{wsl} & 0.135 & 0.210 & 0.173 \\
12 & \textit{clip} & 0.155 & 0.180 & 0.168 \\
13 & \textit{ircsn} & 0.088 & 0.193 & 0.140 \\
14 & \textit{tf} & 0.102 & 0.142 & 0.122 \\
15 & \textit{c3d} & 0.036 & 0.098 & 0.067 \\
\bottomrule
\end{tabular}}
\label{tab:select-2dfeat}
\end{table}

% \begin{table}[ht!]
% \caption{\textbf{Comparing 2D and 3D visual features on the TRECVID 19/20 AVS task}. Training data: MSR-VTT + TGIF.}
% \centering
% \setlength{\tabcolsep}{1.6mm}
% \scalebox{1}{
%     %  \small 
% \begin{tabular}{clrrr}
% \toprule
% \multicolumn{1}{l}{Rank} & Feature & \multicolumn{1}{c}{\textbf{TV19}} & \multicolumn{1}{c}{\textbf{TV20}} & \multicolumn{1}{c}{\textbf{MEAN}} \\
% \hline
% \multicolumn{5}{l}{\textbf{\textit{Model}: SEA(bow, w2v) \cite{tmm21-sea}  }} \\
% 1 & \textit{c3d}& 0.036 & 0.098 & 0.067 \\
% 2 & \textit{tf} & 0.102 & 0.142 & 0.122 \\
% 3 & \textit{ircsn} & 0.088 & 0.193 & 0.140 \\
% 4 & \textit{clip} & 0.155 & 0.180 & 0.168 \\
% 5 & \textit{wsl} & 0.135 & 0.210 & 0.173 \\
% 6 & \textit{rx101-wsl} & 0.148 & 0.208 & 0.178 \\
% 7 & \textit{clip-wsl} & 0.148 & 0.208 & 0.178 \\
% 8 & \textit{rx101-re152-wsl} & 0.159 & 0.208 & 0.184 \\
% 9 & \textit{rx101-re152} & 0.167 & 0.201 & 0.184 \\
% 10 & \textit{rx101-clip} & 0.196 & 0.223 & 0.210 \\
% 11 & \textit{rx101-re152-wsl-clip} & 0.182 & 0.238 & 0.210 \\
% 12 & \textit{rx101-wsl-clip} & 0.183 & 0.239 & 0.211 \\
% 13 & \textit{rx101-re152-clip} & 0.199 & 0.233 & 0.216\\
% \multicolumn{5}{l}{\textbf{\textit{Model}: SEA-clip \cite{ChenHu2021} }} \\
% 14 & \textit{rx101-re152-clip} & 0.199 & 0.249 & 0.224 \\
% 15 & \textit{rx101-wsl-clip} &  0.204 & 0.262 & 0.233\\

% \bottomrule
% \end{tabular}}

% \label{tab:select-2dfeat}
% \end{table}

==> table-select-3dfeat.tex <==

\begin{table}[ht!]
\caption{\textbf{Evaluating the influence of pre-training on the TRECVID 19/20 AVS tasks}. Retrieval model: MAE.}
% ranked by their overall performance in ascending order.Training on MSR-VTT, TGIF and VATEX.
\centering
\begin{tabular}{lrrr}
\toprule

 \textbf{Visual features}  & \multicolumn{1}{c}{\textbf{TV19}} & \multicolumn{1}{c}{\textbf{TV20}} & \multicolumn{1}{c}{\textbf{MEAN}} \\
 \hline
 \multicolumn{4}{l}{\textit{\textbf{Pre-training on MS-COCO:}}} \\
\textit{rx101-wsl-clip-c3d} & 0.203 & 0.339 & 0.271 \\
\textit{rx101-wsl-clip-tf} & 0.205 & 0.313 & 0.259 \\
\textit{rx101-wsl-clip-ircsn} & 0.196 & 0.347 & 0.272 \\

 \multicolumn{4}{l}{\textit{\textbf{Pre-training on GCC:}}} \\
 \textit{rx101-wsl-clip-c3d} & 0.199 & 0.331 & 0.265 \\
\textit{rx101-wsl-clip-ircsn} & 0.203 &0.335 & 0.269 \\
\multicolumn{4}{l}{\textit{\textbf{Pre-training on GCC and MS-COCO:}}} \\
\textit{rx101-wsl-clip-ircsn} & 0.209 & 0.357 & 0.283\\

\bottomrule
\end{tabular}

\label{tab:select-3dfeat}
\end{table}

==> table-select-clip-bnl.tex <==
\begin{table} [htbp!]
\renewcommand{\arraystretch}{1}
\caption{\textbf{Comparing the influence of CLIP and CLIP-bnl on the TRECVID 16-21 AVS tasks}. }

\label{tab:select-clip-bnl}
\centering
 \scalebox{0.63}{
 \begin{tabular}{@{} llrrrrrrrr @{}}
\toprule
\textbf{Model} & \multicolumn{1}{l}{\textbf{TV16}} & \multicolumn{1}{l}{\textbf{TV17}} & \multicolumn{1}{l}{\textbf{TV18}} & \multicolumn{1}{l}{\textbf{TV19}} & \multicolumn{1}{l}{\textbf{TV20}} & \multicolumn{1}{l}{\textbf{TV21}} & \multicolumn{1}{l}{\textbf{MEAN}} \\
\hline
LAFF+CLIP(ViT-B/32)  & 0.259 & 0.35 & 0.189 & 0.238 & 0.359 & 0.353 & 0.291 \\
LAFF+CLIP-bnl & 0.262 & 0.357 & 0.192 & 0.243 & 0.358 & 0.361 & 0.296 \\
 % \hline

\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}



==> table-submmit21.tex <==
\begin{table*} [htbp!]
\renewcommand{\arraystretch}{1}
\caption{\textbf{Performance of our TV21 submissions and two baselines on TRECVID 2016--2021 AVS tasks}.}

\label{tab:avs-submmit21}
\centering
 \scalebox{0.95}{
 \begin{tabular}{@{} llrrrrrrr @{}}
\toprule

\textbf{Submission} & \textbf{Solution} &\textbf{TV16} & \textbf{TV17} &\textbf{TV18} &\textbf{TV19} & \textbf{TV20} & \textbf{TV21}& \textbf{MEAN} \\
 \hline
Run1 & Late fusion (Run3, Run4, CLIP) & \textbf{0.246} & 0.320 & 0.161 & \textbf{0.227} & \textbf{0.366} & \textbf{0.343} & 0.277 \\
Run2 & MEA-rerank & 0.224 & \textbf{0.342} & \textbf{0.168} & 0.224 & 0.361 & 0.340 & \textbf{0.293} \\
Run3 & MEA & 0.223 & 0.342 & 0.167 & 0.223 & 0.361 & 0.340 & 0.292 \\
Run4 & SEA-clip & 0.232 & 0.255 & 0.135 & 0.213 & 0.358 & 0.337 & 0.239 \\
 \hline
 - &CLIP &0.173 	&0.208 	&0.087 	&0.136	&0.161	&0.194 	&0.160 \\
 - & Late fusion (Run3, Run4) & 0.235 & 0.300 & 0.156 & 0.225 & 0.365 & 0.339 & 0.270 \\

\bottomrule
\end{tabular}
 }% end of scalebox
\end{table*}



==> table-submmit22.tex <==
\begin{table*} [htbp!]
\renewcommand{\arraystretch}{1}
\caption{\textbf{Performance of our TV22 submissions on TRECVID 2016--2022 AVS tasks}.}

\label{tab:avs-submmit21}
\centering
 \scalebox{0.9}{
 \begin{tabular}{@{} llrrrrrrrrr @{}}
\toprule

\textbf{Runs} &\textbf{Solution}  &\textbf{TV16} & \textbf{TV17} &\textbf{TV18} &\textbf{TV19} & \textbf{TV20} & \textbf{TV21}&  \textbf{TV22}&\textbf{MEAN} \\
 \hline
Run 1 & Late fusion (LAFF on augmented queries)& \textbf{0.282} & 0.367 & 0.188 & \textbf{0.258} & 0.350 & \textbf{0.359} & 0.248 & 0.293 \\
Run 2 & Late fusion (Run 3,LAFF on narrative queries ) & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \multicolumn{1}{r}{-} & \textbf{0.262} & \multicolumn{1}{r}{-} \\
Run 3 & LAFF w/o w2v and bow & 0.280 & 0.350 & 0.178 & 0.244 & 0.319 & 0.326 & 0.258 & 0.279 \\
Run 4 & LAFF &0.282 & \textbf{0.368} & \textbf{0.197} & 0.255 & \textbf{0.361} & 0.365 & 0.257 & 0.298\\
\hline
{-} &Late fusion (Run 3, Run 4) &0.287	&0.364	&0.193	&0.252	&0.355	&0.356 &0.266&0.296\\
 % \hline

\bottomrule
\end{tabular}
 }% end of scalebox
\end{table*}



% \begin{table*} [htbp!]
% \renewcommand{\arraystretch}{1}
% \caption{\textbf{Performance of our TV22 submissions and two baselines on TRECVID 2016--2021 AVS tasks}.}

% \label{tab:avs-submmit21}
% \centering
%  \scalebox{0.95}{
%  \begin{tabular}{@{} llrrrrrrr @{}}
% \toprule

% \textbf{Submission} & \textbf{Solution} &\textbf{TV16} & \textbf{TV17} &\textbf{TV18} &\textbf{TV19} & \textbf{TV20} & \textbf{TV21}& \textbf{MEAN} \\
%  \hline
% Run1 & Late fusion (Run3, Run4, CLIP) & \textbf{0.246} & 0.320 & 0.161 & \textbf{0.227} & \textbf{0.366} & \textbf{0.343} & 0.277 \\
% Run2 & MEA-rerank & 0.224 & \textbf{0.342} & \textbf{0.168} & 0.224 & 0.361 & 0.340 & \textbf{0.293} \\
% Run3 & MEA & 0.223 & 0.342 & 0.167 & 0.223 & 0.361 & 0.340 & 0.292 \\
% Run4 & SEA-clip & 0.232 & 0.255 & 0.135 & 0.213 & 0.358 & 0.337 & 0.239 \\
%  \hline
%  - &CLIP &0.173 	&0.208 	&0.087 	&0.136	&0.161	&0.194 	&0.160 \\
%  - & Late fusion (Run3, Run4) & 0.235 & 0.300 & 0.156 & 0.225 & 0.365 & 0.339 & 0.270 \\

% \bottomrule
% \end{tabular}
%  }% end of scalebox
% \end{table*}




==> vtt-generation.tex <==

\section{Video-to-Text Description Generation}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=2.1\columnwidth]{mh7.png}
    \caption{\textbf{Proposed solution for video captioning} \cite{mm21gch}. The solution consists of four key steps: 1) scene-level and object-level feature extraction, 2) feature enhancement by multi-head self attention, 3) candidate caption generation by Bottom-Up-Top-Down, and 4) caption reranking by cross-modal matching. The entire network is end-to-to-end trained by reinforcement and adversarial learning, with a BERT based semantic similarity between  generated and reference captions added into the reward and a jointly trained discriminator.}
    \label{fig:vttmodel}
\end{figure*}
In this subtask, participants were asked to automatically generate a natural language sentence to describe the content of a given \emph{unlabeled} video.
%, and without taking into consideration the existence of any annotated descriptions for this video.

\subsection{Approach}
Our solutions are developed on the basis of the classical Bottom-Up-Top-Down (BUTD) model\cite{Anderson2018BottomUpAT}, by improving its encoder and decoder \cite{mm21gch}. The overall architectures is illustrated in Fig. \ref{fig:vttmodel}.




\subsubsection{Multi-Level Video Feature Extraction and Enhancement}

Multi-level visual representation learning is found to be crucial for a comprehensive representation of the video content \cite{tpami21-de,tcsvt2022-rivrl}. In this work, we extract both holistic scene-level features and fine-grained object-level features. Scene-level features are extracted from various pre-trained models such as ResNext\cite{wsl}, CLIP (ViT-B/32)~\cite{2021clip_icml}, TimesFormer\cite{timesformer}, X3D\cite{x3d} and irCSN\cite{ircsn}, as previously used for the AVS task. In order to extract features for salient objects, we propose to apply a pre-trained video object segmentation network, AGNN\cite{agnn}, instead of widely used Faster-RCNN as the object-level feature extractor. To align and enhance the scene- and object- level features, a multi-head self-attention module~(MHSA) is used. 


\subsubsection{Caption Generation Network}

Our caption generation network is based on the widely used Bottom-Up-Top-Down (BUTD) model \cite{Anderson2018BottomUpAT}. In a nutshell, BUTD runs two LSTMs, \ie an attention LSTM (att-LSTM) and a language LSTM (lang-LSTM), in turn. 
To deal with the scene-level and object-level features, we introduce two att-LSTMs. The scene-att-LSTM concentrates on the significance of diverse scene features, while the object-att-LSTM attends the relationship among temporal frames from the object aspect. By applying such dual attention LSTMs, we effectively exploit multi-level visual representation for caption generation.


\begin{table*}[htbp]
\centering
% \setlength{\tabcolsep}{1.2mm}
\caption{\textbf{Our runs in the TRECVID 2021 VTT description generation subtask.} Our best run receives CIDEr-D of 28.8\%.}
\begin{tabular}{lcccc|cccc}
\toprule

\multicolumn{1}{l|}{\multirow{1}{*}{Run}}                     & \specialcell{Feature Extraction \\ \& Enhancement} & \specialcell{Reinforced \\Learning} & \specialcell{Adversarial \\ Learning} & Reranking & Bleu\_4                           & METEOR                             & CIDEr\_D                          & SPICE                             \\ \midrule
\multicolumn{1}{c|}{1}                 & \ding{51}                                 & \ding{51}                  & \ding{55}                    & \ding{55}         & 9.65                              & 27.13                              & 25.3                              & 9.3                               \\
\multicolumn{1}{c|}{2}                 & \ding{51}                                  & \ding{51}                   &     \ding{51}     & \ding{55}         & 9.65                              & 27.02                              & 25.5                              & 9.2                               \\
\multicolumn{1}{c|}{3}                 & \ding{51}                                  & \ding{51}                   & after 5 epoch                   & \ding{55}         & 9.35                              & 27.05                              & 25.4                              & 9.3                               \\ 
\multicolumn{1}{c|}{4}                                     & \textbf{-} & \textbf{-} & \textbf{-}                                                   & \ding{51}         & \textbf{9.88} & \textbf{28.46} & \textbf{28.8} & \textbf{10.3} \\ \bottomrule
\end{tabular}
\label{tab:vtt_result}

\end{table*}



\subsubsection{Reinforced Adversarial Learning}
Towards generating human-like captions, our model is trained in a semantic-reinforced and adversarial manner besides minimizing the cross-entropy loss in word prediction.
Firstly, we adopt a semantic-reinforced training strategy via self-critical sequence training (SCST), which has been proved effective in image and video captioning \cite{selfcritical,selfcritical1,selfcritical2,Anderson2018BottomUpAT}. As for the choice of the rewards for reinforcement learning, previous works use metrics(\eg CIDEr-D\cite{vedantam2015cider}). We further consider a semantic similarity-based reward. In particular, a pre-trained SentenceBert \cite{sentencebert} is used to measure the similarity score between generated captions and corresponding ground truth.
Secondly, we apply a discriminator to estimate how likely the generated captions share the same fluency and language style with the groundtruths. In such an adversarial training manner, the decoder, which can be regarded as a generator, can be optimized jointly with the discriminator towards generating more fluent and human-like captions.


\subsubsection{Caption Reranking by Cross-Modal Matching}

Multiple models are trained with different setups. In order to pick up the best caption from candidate captions generated independently by these models, a retrieval-based caption reranking is conducted \cite{mm2016-v2t}. To be specific, two pretrained video-text matching models, SEA\cite{tmm21-sea} and CLIP (ViT-B/32)~\cite{2021clip_icml}, are utilized to calculate the alignment scores between the given video and each candidate caption. 
Both SEA and CLIP embed the video and captions into a common space, wherein the cross-modal semantic similarity is computed as the cosine similarity between the corresponding embedding vectors. We average the similarity scores from the two models. The caption with the highest score is selected.


\subsection{Submissions}

We use five public datasets for training, including the training split of MSR-VTT \cite{msrvtt}, TGIF \cite{tgif},  VATEX \cite{vatex} and TRECVID VTT 2018-2019 \cite{2019trecvid}. The VTT 2020 training set \cite{2020trecvid} is used for internal evaluation. 
As the effectiveness of feature extraction \& enhancement, caption generation and semantic-reinforced training are separately verified in our previous work\cite{mm21gch}, we start from the internal evaluation of adversarial training. The following four runs are submitted:
\begin{itemize}
    \item \emph{Run 1} is the baseline model, which use merely semantic-reinforced training strategy.

    \item \emph{Run 2} adds adversarial learning based on \emph{Run 1}.

    \item \emph{Run 3} starts adversarial learning after 5 epoch due to the saturation of discriminator. 
    
    \item \emph{Run 4} is the ensemble version via reranking. 
\end{itemize}

Results are shown in Table \ref{tab:vtt_result}. 
Adversarial training  requires further exploration for better generalization, and the ensemble version via reranking shows the most significant improvements. An overview of the VTT Description Generation task benchmark is shown in Fig. \ref{fig:vgg-runs}. Team-wise, our submissions are ranked at the second place among all the submissions.


\begin{figure}[tb!]
\centering
\includegraphics[width=\columnwidth]{vtt2.pdf}
\caption{\textbf{Overview of the TRECVID 2021 VTT Description Generation benchmark evaluation}.}
\label{fig:vgg-runs}
\end{figure}












==> vtt.tex <==

% For video-to-text matching, we participate in both the Matching and Ranking subtask and Description Generation subtask. 


\subsection{Matching and Ranking}
Given a video, participants were asked to rank a list of pre-defined candidate sentences in terms of their relevance with respect to the given video. In the 2019 edition, the test video set consists of 2,054 videos where 1044 videos are collected from Twitter Vine and 1010 videos are from Flickr. Five sentence sets are provided by the task organizers, denoted as setA, setB, setC, setD and setE. Each sentence set has 2,054 sentences. 

\subsubsection{Approach}

\begin{figure*}[tb!]
\centering\includegraphics[width=1.8\columnwidth]{vtt-matching}
\caption{Conceptual diagram of our improved dual encoding network for the Video-to-Text Matching and Ranking task.}\label{fig:vtt-matching}
\end{figure*}

Dual Encoding~\cite{cvpr19-zevr} is used.  Additionally, we improve the dual encoding network by including the BERT encoder as used in our AVS runs. The BERT feature is concatenated with the global, local and temporal features extracted by multi-level encoding, see Fig. \ref{fig:vtt-matching}.


We train models on a combined set of MSR-VTT \cite{msrvtt}, MSVD \cite{msvd} and TGIF \cite{tgif}, with hyper-parameters tuned on the TRECVID 2016 VTT training set. 


\subsubsection{Submissions}

We submit the following four runs:
\begin{itemize}
    \item \emph{Run 1} is the original dual encoding model using the ResNeXt-101 feature. 

    \item \emph{Run 2} is the improved dual encoding model with the BERT features as the extra input. The ResNeXt-101 feature is used.

    \item \emph{Run 3} equally combines six models, among with three models are based on \emph{Run 1} with their video feature varies. That is, ResNeXt-101 feature, ResNet-152 feature, and the concatenate of ResNeXT-152 and ResNeXt-101 features. The other three models are based on \emph{Run 2}, using the same three video features.

    \item \emph{Run 4} combines \emph{Run 3} and other two W2VV++ variants. One is original W2VV++ model (\emph{Run 4} in AVS task), the other is W2VV++ with BERT encoder (\emph{Run 3} in AVS task). 
\end{itemize}


Table \ref{tab:perf-on-test} summaries our results in the TRECVID 2019 VTT matching and ranking subtask. \emph{Run 2}, by including the BERT features, outperforms \emph{Run 2}. \emph{Run 3} combing 6 models gives the best performance.



\begin{table} [tb!]
\renewcommand{\arraystretch}{1.2}
\caption{\textbf{Our runs in the TRECVID 2019 VTT matching and ranking subtask}. 
% Our re-evaluation, using the official ground truth, is able to exactly re-produce the numbers for setA, setB and setC, yet the new numbers on setD and setE appear to be much higher than those returned by TRECVID.
}
\label{tab:perf-on-test}
\centering
 \scalebox{0.99}{
     \small \begin{tabular}{@{} c*{6}{c} @{}}
\toprule
         % && \multicolumn{5}{c}{\textbf{Official Evaluation}} &  & \multicolumn{2}{c}{\textbf{Our Re-Evaluation}} \\
         % \cmidrule(r){3-7}  \cmidrule(r){9-10} 
\textbf{Ours}         && setA & setB & setC & setD & setE  \\
\midrule
% \cmidrule(r){1-10} \cmidrule(r){12-20}
%\hline
% \midrule
         \emph{Run 1}       && 0.432 & 0.442 & 0.429 & 0.437 & 0.441 \\
         \emph{Run 2}       && 0.436 & 0.443 & 0.444 & 0.447 & 0.446 \\
         \emph{Run 3}       && \textbf{0.474} & \textbf{0.480} & \textbf{0.474} & \textbf{0.487} & \textbf{0.481} \\
         \emph{Run 4}       && 0.471 & \textbf{0.480} & 0.470 & 0.484 & 0.477 \\
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}




% \begin{figure*}[tb!]
% \centering
% %
%  \subfigure[setA]{
% \noindent\includegraphics[width=1.8\columnwidth]{draw_vtt/vtt_setA_v2}
% \label{fig:tv17-setA}
% }
% %
%  \subfigure[setB]{
% \noindent\includegraphics[width=1.8\columnwidth]{draw_vtt/vtt_setB_v2}
% \label{fig:tv17-setB}
% }
%  \subfigure[setC]{
% \noindent\includegraphics[width=1.8\columnwidth]{draw_vtt/vtt_setC_v2}
% \label{fig:tv17-setC}
% }
% %
% %  \subfigure[setD]{
% % \noindent\includegraphics[width=1.9\columnwidth]{draw_vtt/vtt_setD_v2}
% % \label{fig:tv17-setD}
% % }
% % %
% %  \subfigure[setE]{
% % \noindent\includegraphics[width=1.9\columnwidth]{draw_vtt/vtt_setE_v2}
% % \label{fig:tv17-setE}
% % }
% %
% \caption{\textbf{Overview of the TRECVID 2018 video-to-text matching and ranking task benchmark on setA, setB and setC}, all runs ranked according to MIR. We were the best overall performer.}
%  \label{fig:vtt-results}
% \end{figure*}


% \begin{figure*}[tb!]
% \centering
% %
% %  \subfigure[setA]{
% % \noindent\includegraphics[width=1.8\columnwidth]{draw_vtt/vtt_setA_v2}
% % \label{fig:tv17-setA}
% % }
% % %
% %  \subfigure[setB]{
% % \noindent\includegraphics[width=1.8\columnwidth]{draw_vtt/vtt_setB_v2}
% % \label{fig:tv17-setB}
% % }
% %  \subfigure[setC]{
% % \noindent\includegraphics[width=1.8\columnwidth]{draw_vtt/vtt_setC_v2}
% % \label{fig:tv17-setC}
% % }

%  \subfigure[setD]{
% \noindent\includegraphics[width=1.9\columnwidth]{draw_vtt/vtt_setD_v2}
% \label{fig:tv17-setD}
% }
% %
%  \subfigure[setE]{
% \noindent\includegraphics[width=1.9\columnwidth]{draw_vtt/vtt_setE_v2}
% \label{fig:tv17-setE}
% }

% \caption{\textbf{Overview of the TRECVID 2018 video-to-text matching and ranking task benchmark on setD and setE}, all runs ranked according to MIR. We were the best overall performer.}
%  \label{fig:vtt-results-2}
% \end{figure*}










